Adversarial Training and Provable Robustness: A Tale of Two Objectives

We propose a principled framework that combines adversarial training and provable robustness verification for training certifiably robust neural networks. We formulate the training problem as a joint optimization problem with both empirical and provable robustness objectives and develop a novel gradient-descent technique that can eliminate bias in stochastic multi-gradients. We perform both theoretical analysis on the convergence of the proposed technique and experimental comparison with state-of-the-arts. Results on MNIST and CIFAR-10 show that our method can consistently match or outperform prior approaches for provable l infinity robustness. Notably, we achieve 6.60% verified test error on MNIST at epsilon = 0.3, and 66.57% on CIFAR-10 with epsilon = 8/255.

==> Makefile <==
.DEFAULT_GOAL := default

# default goal
default: pdf clean

## Create PDF
pdf:
#	latex paper.tex
#	bibtex paper.aux
#	latex paper.tex
#	latex paper.tex
#	dvips paper.dvi -o paper.ps -t letter -Ppdf -G0
#	ps2pdf paper.ps
	pdflatex paper.tex
	bibtex paper.aux
	pdflatex paper.tex
	pdflatex paper.tex
	pdflatex paper.tex

## Cleanup build files
clean:
	rm -rf paper.log paper.out paper.aux paper.blg paper.bbl paper.bcf paper.run.xml paper.dvi paper.ps

## Show this help screen
help:
	@printf "Available targets\n\n"
	@awk '/^[a-zA-Z\-\_0-9]+:/ { \
		helpMessage = match(lastLine, /^## (.*)/); \
		if (helpMessage) { \
		helpCommand = substr($$1, 0, index($$1, ":")-1); \
		helpMessage = substr(lastLine, RSTART + 3, RLENGTH); \
		printf "%-30s %s\n", helpCommand, helpMessage; \
		} \
		} \
		{ lastLine = $$0 }' $(MAKEFILE_LIST)

